Structural Insights and an IP-based Solution Method for Patient-to-room Assignment under Consideration of Single Room Entitlements

Patient-to-room assignment (PRA) is a scheduling problem in decision support for hospitals. It consists of assigning patients to rooms according to certain objectives, e.g., avoiding transfers and respecting single-room requests. This work presents combinatorial insights about the feasibility of PRA and about the assignment of patients to single rooms. We further compare different IP-formulations for PRA as well as the influence of different objectivs on the runtime. Based on these results, we develop a fast IP-based solution approach which obtains high quality solution. The applicability is verified through a computational study with instances derived from real-world data. Results indicate that large, real world instances can be solved to a high degree of optimality within (fractions of) seconds.

==> Images/tikz_estimatedlos.tex <==
\begin{tikzpicture}

\draw[->] (-3, 0) -- (4.2, 0) node[right] {$\gamma$};
\draw[->] (0, -3) -- (0, 4.2) node[above] {$e_p(\gamma)$};

\caption{Patient with expected length of stay $5.5$ days and actual length of stay $3$ days.}

\end{tikzpicture}

\begin{tikzpicture}

\draw[->] (-3, 0) -- (4.2, 0) node[right] {$\gamma$};
\draw[->] (0, -3) -- (0, 4.2) node[above] {$e_p(\gamma)$};

\caption{Patient with expected length of stay $2$ days and actual length of stay $7$ days.}

\end{tikzpicture}



==> Images/tikz_modelcomby_static.tex <==
\begin{figure}[ht!]
    \centering
    \scalebox{0.5}{
        
\begin{tikzpicture}[node distance=2cm,every label/.style={align=left}]
    
    % Styles
    \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=RWTHred!50]

    \tikzstyle{process} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=RWTHorange]
    
    \tikzstyle{decision} = [diamond, minimum width=2cm, minimum height=2cm, text centered, draw=black, fill=RWTHmaygreen]
    
    \tikzstyle{YN} = [minimum width=0cm, minimum height=0cm, text centered]

    \tikzstyle{arrow} = [thick,->,>=stealth]
        
    % Actual Figure
    \node (initialisation) [startstop] {Initialisation};
    \node (feasibility) [decision,right of= initialisation,xshift=1.5cm] {Feasible?};
    
    \draw [arrow] (initialisation) -> (feasibility);
    
    \node (yes0) [YN,below of=feasibility, yshift=0.9cm,xshift=0.4cm] {Yes};
    \node (no0) [YN,right of=feasibility, yshift=-0.35cm,xshift=-0.2cm] {No};
    
    % N Step
    \node (N) [process, below of=feasibility] {N};
    \node (N_eval) [decision, right of=N, xshift=1cm] {Optimal?};
    
    \draw [arrow] (feasibility) -- (N);
    \draw [arrow] (N) -- (N_eval);

    \node (no1) [YN,below of=N_eval, yshift=1.6cm,xshift=1.4cm] {No};
    \node (yes1) [YN,above of=N_eval, yshift=-0.35cm,xshift=0.4cm] {Yes};
    
    % C Step
    \node (C) [process, right of=N_eval, xshift=1cm] {C};
    \node (C_eval) [decision, right of=C, xshift=1cm] {Feasible?};
    
    \draw [arrow] (N_eval) -- (C);
    \draw [arrow] (C) -- (C_eval);

    \node (no2) [YN,below of=C_eval, yshift=1.6cm,xshift=1.4cm] {No};
    \node (yes2) [YN,above of=C_eval, yshift=-0.35cm,xshift=0.4cm] {Yes};
    
    % E Step
    \node (E) [process, right of=C_eval, xshift=1cm] {E};

    \node (terminate) [startstop, above of=E,yshift=0cm] {Terminate};
    
    \draw [arrow] (C_eval) -- (E);
    \draw [arrow] (E) -> (terminate);
    \draw [arrow] (C_eval) |- (terminate);
    \draw [arrow] (N_eval) |- (terminate);
    
    \draw [arrow] (feasibility) -> (terminate);

    \draw[dashed] (13.5,-0.8) rectangle (17.5,-3.5);

\end{tikzpicture}

}
    \caption{Implemented structure for solving the static PRA. The dotted part is only required in theory, but not executed in practise.}
    \label{fig:programstructure}
\end{figure}

==> sections/04_Model_short.tex <==
\section{IP Formulation}
In this section, we present two integer programms for PRA.
The first IP is a general 
These IPs are the result of an extensive computational study where we evaluated the computational performance of 


\begin{maxi!}
{}{(-\transobj,\privobj)}{}{}
\label{IP:H}
\tag{H}
\addConstraint{\sum_{r \in  R} x_{prt}}{= 1}{\forall p \in P}
\addConstraint{x_{prt} - x_{pr(t+1)}}{\leq \delta_{prt}}{\forall r\in\R,\ p\in\P, \arr_p\leq t < \dis_p-1}
\addConstraint{s_{prt}}{\leq x_{pr}}{\forall p\in P^*, r\in R, t \in T}
\addConstraint{\sum_{p\in P^\mathrm{f}(t)} x_{prt} + \sum_{p\in P^\mathrm{f}\cap P^*(t)} (c_r-1)s_{prt}}{\leq c_r g_{rt}\quad}{\forall t\in T,\ r\in R}
\addConstraint{\sum_{p\in P^\mathrm{m}(t)} x_{prt} + \sum_{p\in P^\mathrm{m}\cap P^*(t)} (c_r-1)s_{prt}}{\leq c_r (1-g_{rt})\quad}{\forall t\in T,\ r\in R}
\addConstraint{x_{prt},g_{rt},m_{rt},s_{prt}}{\in\{0,1\}}{\forall p\in P, r\in R, t \in T}
\end{maxi!}

\begin{maxi!}
{}{\privobj}{}{}
\label{IP:O}
\tag{O}
\addConstraint{\sum_{r \in  R} x_{pr}}{= 1}{\forall p \in P}
\addConstraint{s_{prt}}{\leq x_{pr}}{\forall p\in P^*, r\in R, t \in T}
\addConstraint{\sum_{p\in P^\mathrm{f}(t)} x_{pr} + \sum_{p\in P^\mathrm{f}\cap P^*(t)} (c_r-1)s_{prt}}{\leq c_r g_{rt}\quad}{\forall t\in T,\ r\in R}
\addConstraint{\sum_{p\in P^\mathrm{m}(t)} x_{pr} + \sum_{p\in P^\mathrm{m}\cap P^*(t)} (c_r-1)s_{prt}}{\leq c_r (1-g_{rt})\quad}{\forall t\in T,\ r\in R}
\addConstraint{x_{pr},g_{rt},m_{rt},s_{prt}}{\in\{0,1\}}{\forall p\in P, r\in R, t \in T}
\end{maxi!}

\begin{maxi!}
{}{0}{}{}
\label{IP:P}
\tag{P}
\addConstraint{\sum_{r \in  R} x_{pr}}{= 1}{\forall p \in P}
\addConstraint{s_{prt}}{\leq x_{pr}}{\forall p\in P^*, r\in R, t \in T}
\addConstraint{\sum_{p\in P^\mathrm{f}(t)} x_{pr} + \sum_{p\in P^\mathrm{f}\cap P^*(t)} (c_r-1)s_{prt}}{\leq c_r g_{rt}\quad}{\forall t\in T,\ r\in R}
\addConstraint{\sum_{p\in P^\mathrm{m}(t)} x_{pr} + \sum_{p\in P^\mathrm{m}\cap P^*(t)} (c_r-1)s_{prt}}{\leq c_r (1-g_{rt})\quad}{\forall t\in T,\ r\in R}
\addConstraint{\sum_{p\in P^*}\sum_{r \in R} s_{prt}}{\geq s^{\mathrm{max}}_t}{\forall t \in T}
\addConstraint{x_{pr},g_{rt},m_{rt},s_{prt}}{\in\{0,1\}}{\forall p\in P, r\in R, t \in T}
\end{maxi!}

